Rate Allocation and Content Placement in Cache Networks

We introduce the problem of optimal congestion control in cache networks, whereby \emph{both} rate allocations and content placements are optimized \emph{jointly}. We formulate this as a maximization problem with non-convex constraints, and propose solving this problem via (a) a Lagrangian barrier algorithm and (b) a convex relaxation. We prove different optimality guarantees for each of these two algorithms; our proofs exploit the fact that the non-convex constraints of our problem involve DR-submodular functions.

==> oldendingofthm1.tex <==
Finally, by Assumption~\ref{assm:unbounded}, at least one utility function is unbounded from above. Therefore, we can show in the following lemma that the optimal objective value grows without any bound as we increase the link capacities and demand rates.
\begin{lem}
\label{lem:fminf}
If Assumption~\ref{assm:unbounded} holds, we have 
\begin{equation*}
     \lim_{m \to \infty} F( \boldsymbol{R}^* (m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) ) = \infty.
\end{equation*}
\end{lem}

Lemma~\ref{lem:fminf}, proved in Appendix~\ref{append:ProofOfLemFminF},  implies that there exists a $m_0 > 0$ such that 
\begin{equation} \label{equ:fmpos}
F( \boldsymbol{R}^* (m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) ) > 0 \quad \forall m \geq m_0.
\end{equation}

Given \eqref{equ:fmpos}, we can divide both sides of \eqref{equ:greaterwithm} by $F( \boldsymbol{R}^* (m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) ),$ for all $m \geq m_0$. We then obtain \begin{align} \tiny
    &\frac{ F( \hat{\boldsymbol{R}}(m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) )}{F( \boldsymbol{R}^* (m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) )} \geq 1 - \nonumber \\
    & \frac{\theta}{F( \boldsymbol{R}^* (m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) )} \sum_{(b,a) \in \mathcal{E}} n_{ab} \frac{\left(\sum_{(i,p) : (a,b) \in p} \bar{\lambda}_{(i,p)} - C_{ba}\right)}{C_{ba}}.
     \label{equ:fraction}
\end{align}

Finally, by Lemma~\ref{lem:fminf} and \eqref{equ:fraction}, we have
\begin{equation*}
    \lim_{m\to\infty} \frac{F( \hat{\boldsymbol{R}}(m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) )}{F( \boldsymbol{R}^* (m\boldsymbol{C},m\bar{\boldsymbol{\lambda}}) )} = 1,
\end{equation*}
and this concludes the proof.

==> table.tex <==

\begin{table}[!t]
\begin{footnotesize}
\caption{Notation Summary}%\vspace*{-10mm}
\begin{tabular}{cp{0.7\columnwidth}}
\hline
\multicolumn{2}{c}{\textbf{Notational Conventions}}\\
\hline
$\mathbb{R}$ & Set of real numbers \\
$\mathbb{R}_+$ & Set of real numbers $x \in \mathbb{R}$, s.t. $x \geq 0$ \\
$\mathbb{N}$ & Set of natural numbers  \\
$\vee$ &  Coordinate-wise maximum \\
$\wedge$ & Coordinate-wise minimum\\
$[K]$ & Set of numbers $\{ 1,\dots, K \}$, for $K \in \mathbb{N}$\\
\hline
\multicolumn{2}{c}{\textbf{Cache Networks}}\\
\hline
$G(\mathcal{V},\mathcal{E})$ & Network graph, with nodes $\mathcal{V}$ and links $\mathcal{E}$\\
%$k_p(v)$ & position of node $v$ in path $p$\\
$C_{ab}$ & Link capacity for $(a,b)$  (in number of items per second)\\
$\boldsymbol{C}$& $|\mathcal{E}|$-dimensional vector of $C_{ab}$, for $(a,b) \in \mathcal{E}$  \\
$c_v$ & Node capacity of $v\in V$ (in number of items)\\
$\itemcat$ & Item catalog \\
$\requestset$ & Set  of requests $\requestindex=(i,p)$, with $i \in \itemcat$ and $p\subseteq \mathcal{V}$ a path \\
%$(i,p)$ & kjk \\
$\bar{\lambda}_{\requestindex}$ & Demand rate of request $\requestindex \in \requestset$\\
$\lambda_{\requestindex}$ & Allocated rate of request $\requestindex \in \requestset$, in $[0,\bar{\lambda}_{\requestindex}]$\\
$r_{\requestindex}$ & Residual rate of request $\requestindex \in \requestset$, in $[0,\bar{\lambda}_{\requestindex}]$\\
%$(i,p)$& Request consisting of the item $i$ and the path $p$\\
$\mathcal{S}_i$ & Set of designated sources of $i\in \itemcat$\\
$x_{vi}$ & Cache indicator variable, indicating whether $v\in \mathcal{V}$ is storing $i\in\itemcat$, in $\{0,1\}$ \\
$y_{vi}$ & Cache allocation variable, indicating probability that  $v\in \mathcal{V}$ is storing $i\in\itemcat$, in $[0,1]$ \\
%$\mathbf{x}$ & Placement vector of $x_{vi}$s, in $\{0,1\}^{|V||\catalog|}$\\ %/relaxed variable $x_{vi}$\\
%$\bm{\lambda}$ & Vector of arrival rates $\lambda^r$, $r\in \demand$\\
%$\lambda_e^r$ & Arrival rate of class $r$ responses over edge $e\in E$\\
%$\rho_e$ & Load on edge $e\in E$\\
%$Q$ & Set of request sources\\
$\boldsymbol{Y}$ & (cache allocation strategy) $|\mathcal{V}| |\itemcat|$-dimensional vector  of  $y_{vi}$, for $v \in \mathcal{V}$ and $i \in \itemcat$ \\
$\boldsymbol{\lambda}$ & (rate allocation strategy) $|\requestset|$-dimensional vector of $\lambda_{\requestindex}$ , for $\requestindex \in \requestset$ \\
$\bar{\boldsymbol{\lambda}}$&   $|\requestset|$-dimensional vector of $\bar{\lambda}_{\requestindex}$, for $\requestindex \in \requestset$\\
$\boldsymbol{R}$ & $|\requestset|$-dimensional vector of $r_{\requestindex}$ , for $\requestindex \in \requestset$ \\
$F(\boldsymbol{R})$ & Objective function (equal to aggregate utility $U(\boldsymbol{\lambda})$)\\
$\mathcal{D}_1$ & Set of feasible $(\boldsymbol{Y},\boldsymbol{R})$ for \textsc{UtilityMax}\\
$g_{ba}(\cdot)$ & Functions defined in \eqref{equ:gba} and used in the constraints \eqref{const:link}\\
$g_{v}(\cdot)$ & Functions defined in \eqref{equ:gv} and used in the constraints \eqref{const:cache}\\
\hline 
\multicolumn{2}{c}{\textbf{Lagrangian Barrier Method}}\\
\hline
$\Psi(\cdot)$ &Lagrangian barrier function \eqref{equ:psi} \\
$\mu_{ba}, \gamma_v$ & Lagrange multiplier estimates \\
$s_{ba}, s_v$   & Shifts \\
$\omega_k$ & Accuracy of the solution at the $k$-th iteration\\
$\mathcal{B}$ & Box constraints \eqref{const:boxfory} and \eqref{const:boxforlambda}\\
%\hline 
%\multicolumn{2}{c}{\textbf{Theorem}~\ref{thm:assymptotic}}\\
%\hline
$\hat{\boldsymbol{Y}}(\boldsymbol{C},\bar{\boldsymbol{\lambda}})$ & $\boldsymbol{Y}$ at limit point of the sequence generated by Alg.~\ref{alg:findKKT} for a problem with link capacities $\boldsymbol{C}$ and demand rates  $\boldsymbol{\lambda}$\\
 $\hat{\boldsymbol{R}}(\boldsymbol{C},\bar{\boldsymbol{\lambda}})$ &$\boldsymbol{R}$ at limit point of the sequence generated by Alg.~\ref{alg:findKKT} for a problem with link capacities $\boldsymbol{C}$ and demand rates  $\boldsymbol{\lambda}$\\
$\boldsymbol{Y}^*(\boldsymbol{C},\bar{\boldsymbol{\lambda}})$  & Optimal $\boldsymbol{Y}$ for  \textsc{UtilityMax} with link capacities $\boldsymbol{C}$ and demand rates  $\boldsymbol{\lambda}$\\
$\boldsymbol{R}^*(\boldsymbol{C},\bar{\boldsymbol{\lambda}})$ & Optimal $\boldsymbol{R}$ for  \textsc{UtilityMax} with link capacities $\boldsymbol{C}$ and demand rates  $\boldsymbol{\lambda}$\\
%$m$& Coefficient with which the link capacities and demand rates are scaled \\
$n_{ab}$ &Number of paths passing through the link $(a,b)$\\
$\theta$ & The constant in the  logarithmic diminishing  return (Def.~\ref{def:logDR})\\ 
\hline
\multicolumn{2}{c}{\textbf{Convex Relaxation}}\\
\hline
$\mathcal{D}_2$ & Set of feasible $(\boldsymbol{Y},\boldsymbol{R})$ for \textsc{ConvexUtilityMax}\\
$\mathcal{D}_3$ & Set of feasible $(\boldsymbol{Y},\boldsymbol{R})$ for tighter version of  \textsc{UtilityMax}\\
$\tilde{g}_{ba}$ & Concave relaxation of $g_{ba}$ defined in \eqref{eq:gtilde}\\
$C_{ba}'$ & Link capacities defined \eqref{eq:cba_prime}\\
$\boldsymbol{Y}^{**}_{\boldsymbol{C}}$& Optimal $\boldsymbol{Y}$ for  \textsc{ConvexUtilityMax} with link capacities $\boldsymbol{C}$  \\
 $ \boldsymbol{R}^{**}_{\boldsymbol{C}}$ & Optimal $\boldsymbol{R}$ for  \textsc{ConvexUtilityMax} with link capacities $\boldsymbol{C}$ \\
\hline
\hline

\end{tabular}
\vspace*{-2em}
\end{footnotesize}
\end{table}

%%%%%%%%%%%%%%%%


==> techback.tex <==
%\subsection{Constrained Optimization and Optimality Conditions} \label{subsec:constrainedopt}
Consider a general optimization problem of the following form:
\begin{subequations}\label{eq:general}
\begin{align}
    \text{Maximize} \quad &f(\boldsymbol{x})\\
    \text{Subj. to} \quad & g_j(\boldsymbol{x}) \geq 0 \quad j = 1, \dots, r \\
    & h_i(\boldsymbol{x}) = 0 \quad i = 1, \dots, m,
\end{align}
\end{subequations}
where $f : \mathbb{R}^n \rightarrow \mathbb{R}$, $g_j: \mathbb{R}^n \rightarrow \mathbb{R}, ~ j = 1, \dots, r$, and $h_i : \mathbb{R}^n \rightarrow \mathbb{R}, ~ i=1,\dots,m$ are continuously differentiable functions. Here we provide a statement of the most common first-order necessary optimality condition known as \emph{KKT} condition. First let us define a regular point:
\begin{defn}\emph{Regular point}:
If the gradient of equality constraints and active inequality constraints are linearly independent at $\boldsymbol{x}^*$, then $\boldsymbol{x}^*$ is called a regular point. 
\end{defn}
Now, let us formally define \emph{Karush-Kuhn-Tucker} (KKT) points which we use extensively throughout this paper and in stating optimality conditions: 
\begin{defn}\label{def:KKT}
A point $\boldsymbol{x}^*\in \mathbb{R}^n$ is called a KKT point for Problem~\eqref{eq:general} if there exist \emph{Lagrangian variables} $\boldsymbol{\nu}^* \in \mathbb{R}^m$ and $\boldsymbol{\mu}^* \in \mathbb{R}^r$, such that:
\begin{subequations}\label{KKTCondition}
\begin{align*}
    & \nabla_{x}L(\boldsymbol{x}^*, \boldsymbol{\mu}^*, \boldsymbol{\nu}^*) = 0 \\
    &h_i(\boldsymbol{x}^*) = 0 \quad \forall i \in \{1, \dots, m\} \\
    &g_j(\boldsymbol{x}^*) \geq 0 \quad \forall j \in \{1, \dots, r\} \\
    &\mu_j^* \geq 0 \quad \forall j \in \{1, \dots, r\} \\
    &\mu_j^* g_j(\boldsymbol{x}^*) = 0 \quad \forall j \in\{1, \dots, r\}.
\end{align*}
\end{subequations}
where $L(\boldsymbol{x}, \boldsymbol{\mu}, \boldsymbol{\nu}) \triangleq f(\boldsymbol{x}) + \sum_i \nu_i h_i(\boldsymbol{x}) + \sum_j \mu_j g_j(\boldsymbol{x})$ is called the \emph{Lagrangian function}.
\end{defn}

\begin{prop} (First-order KKT Necessary Conditions)
Let $\boldsymbol{x}^*$ be a local minimum of Problem~\eqref{eq:general}, and assume $\boldsymbol{x}^*$ is regular. Then $\boldsymbol{x}^*$ is a KKT point.
\end{prop}
Using the second derivatives of the Lagrangian function, we can state the sufficient condition for optimality.
\begin{prop} (Second-order Sufficiency Conditions)
Assume $f$, $g_j, ~\forall j=1, \dots, r$, and $h_i,~\forall i=1, \dots,m$ are twice continuously differentiable, and $\boldsymbol{x}^*$ is a KKT point with corresponding Lagrange variables $\boldsymbol{\mu}^*$ and $\boldsymbol{\nu}^*$. In addition let 
\begin{equation*}
    \boldsymbol{V}^T \nabla^2_{xx}L(\boldsymbol{x}^*, \boldsymbol{\mu}^*, \boldsymbol{\nu}^*) \boldsymbol{V} <0,
\end{equation*}
for all $\boldsymbol{V} \neq 0$ such that
\begin{align*}
    \nabla h_i(\boldsymbol{x}^*)^T \boldsymbol{V} = 0, ~ \forall i = 1, \dots, m, \\
    \nabla g_j(\boldsymbol{x}^*)^T \boldsymbol{V} = 0, ~ \forall j \in A(\boldsymbol{x}^*).
\end{align*}
In addition assume we have strict complementary slackness, i.e.,
\begin{equation*}
    \mu_j > 0 \quad \forall j \in A(\boldsymbol{x}^*)
\end{equation*}
where $A(\boldsymbol{x}^*)$ is set of active inequality constraints in $\boldsymbol{x}^*$, i.e.,
\begin{equation*}
    A(\boldsymbol{x}^*) \triangleq \{j~|~g_j(\boldsymbol{x}^*) = 0 \}
\end{equation*}
Then $\boldsymbol{x}^*$ is a strict local maximum of Problem~\eqref{eq:general}.
\end{prop}

For further information on other forms of necessary and sufficient conditions for optimality, refer to the book by Bertsekas \cite{bertsekas1999nonlinear}.


